Algorithmic Techniques for Necessary and Possible Winners

We investigate the practical aspects of computing the necessary and possible winners in elections over incomplete voter preferences. In the case of the necessary winners, we show how to implement and accelerate the polynomial-time algorithm of Xia and Conitzer. In the case of the possible winners, where the problem is NP-hard, we give a natural reduction to Integer Linear Programming (ILP) for all positional scoring rules and implement it in a leading commercial optimization solver. Further, we devise optimization techniques to minimize the number of ILP executions and, oftentimes, avoid them altogether. We conduct a thorough experimental study that includes the construction of a rich benchmark of election data based on real and synthetic data. Our findings suggest that, the worst-case intractability of the possible winners notwithstanding, the algorithmic techniques presented here scale well and can be used to compute the possible winners in realistic scenarios.

==> tex_files/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> tex_files/_exp.tex <==
\section{Experimental Evaluation}
\label{sec:exp}

All experiments were carried out on an Intel(R) Xeon(R) CPU E5-2680 v3 @ 2.50GHz, with 412 GB of RAM, 20 hyper-threaded cores running 2 threads per core, running Ubuntu 16.04.6 LTS. We used Python 3.5 for our implementation, and Gurobi v8.1.1 ~\cite{gurobi_2019} for solving the ILP instances of the possible winner problem.  We used both real and synthetic datasets, described below.

\subsection{Experimental Datasets and Scoring Rules}\label{sec:exp:data}  

\paragraph{Real datasets}
We used the following two real datasets. 

{\em travel:} The Google Travel Review Ratings datasets~\cite{renjith2018evaluation} consists of average ratings (each a non-integer between 1 and 5) issued by 5,456 users for up to 24 travel categories in Europe.  For each user, as we create a set of preference pairs such that items in each pair have different ratings (no tied pairs), there cannot be any cycles in the set of preference pairs corresponding to a given user. Also, we do not include the categories in the ranking that were not rated by the given user.

%- The travel dataset consists of average of each user's ratings (non-integers between 1 and 5) issued by 5,456 users for 24 travel categories in Europe. For each user, we create a set of preference pairs such that items in each pair have different ratings (no tied pairs). Because preferences are derived from ratings issued by individual users, there cannot be any cycles in the set of preference pairs corresponding to a given user. 

%- the rating given by a user to a category is an average of multiple ratings given by that user to different places falling under that category. 

%- there are categories with missing ratings (rating of 0 means no rating was given, and does not mean that a rating of 0 was given). These 0 ("missing") ratings are what actually make this dataset a type of partial preference, and hence, interesting. In short, these categories with 0 ratings can take any rank in the completions as we have no information about them.
{\em dessert:} We crowdsourced a dataset of user preferences over pairs of eight desserts, with a total of 228 users and up to 28 pair-wise judgments per user. {\colorThree For each pairs, users indicated their confidence in their choice, which enables us to create several profile, depending on the confidence threshold we choose. With a high confidence threshold, we keep a few pairs and obtain a sparse profile, and with a low confidence threshold, we obtain a very dense profile.

}

\begin{figure}[t]
  \centering
  \begin{tabular}{c @{} c }
  \hspace{-3mm}
  \hspace{-2mm} \includegraphics[trim=0 0 0 0, clip, scale=.4750]{figures/ACM_TDS/partitioned/2-(a)-part.pdf} &
  \includegraphics[trim=0 0 0 0, clip, scale=.4750]{figures/ACM_TDS/partitioned/2-(b)-part.pdf}\\
  \small (a) 100 candidates & \small (b) 10,000 voters
  
  \end{tabular} 
  \vspace{-0.25cm}
  \caption{(a) Running time of the optimized algorithm and (b) speedup factor of the optimized algorithm over the baseline to compute the set of {\bf necessary winners} on \textbf{plurality} scoring rule.}
  \label{fig:NW_plurality}
\end{figure}

\paragraph{Synthetic datasets} \julia{Working on this}

\paragraph{Scoring rules}

We evaluated the performance of our techniques to compute necessary  and possible winners for three positional scoring rules:  {\em plurality}, {\em $2$-approval}, and {\em Borda}. For necessary winners under any of these rules, we implemented an optimized version of the polynomial-time algorithm by Xia and Conitzer \cite{DBLP:journals/jair/XiaC11}, as described in Section \ref{sec:nw}.  For possible winners under the plurality rule, we implemented an optimized version of the polynomial-time algorithm by Betzler and Dorn, as described in Section \ref{sec:pw-betzler-dorn}. 
 For  possible winners under $2$-approval and Borda, we used the reduction to ILP and subsequent optimizations, as described in Sections \ref{pw-ilp}-\ref{sec:possible:threephase}.
The use of this method on the %\rsmm
RSM Mix datasets and under any of these rules is justified because such datasets may contain arbitrary partial orders.  On the partial chain datasets and the \PWPV~datasets under Borda, the use of this method
  is justified because computing possible winners under the Borda rule remains NP-hard (Theorems \kunal{add theorem for partial chain} and \ref{kenig-thm}, respectively (Table~\ref{tab:results})). \st{, even when the partial profiles are restricted to be partial chain or restricted to be \PWPV.}
Finally,  as mentioned in \st{Section} \ref{section:pw-k} Theorem~\ref{kenig-thm}, computing possible winners under $2$-approval is in PTIME on \PWPV~datasets, but not known to be in PTIME on partial chain datasets. We still opted to use the three-phase computation (Section~\ref{sec:possible:threephase}) so that we have a unified set of experimentals across the rules and the datasets. \colorOne We finally measure the efficiency of three-phase computation as compared to known polynomial time algorithms. \colorTwo

\begin{figure}[t]
  \centering
  \begin{tabular}{c @{} c }
  %\hspace{-3mm}
  %\includegraphics[scale=.4750]{figures/ECAI/NW_2app/(c)_m_final.pdf}
  %\hspace{-2mm} &
  %\includegraphics[trim=0 0 0 0, clip, scale=.4750]{figures/ECAI/NW_2app/(c)_speedup_n_final.pdf}\\
  %\small (a) 100 candidates & \small (b) 10,000 voters\\
  \hspace{-3mm}\includegraphics[scale=.4750]{figures/ACM_TDS/partitioned/3-(a)-part.pdf}
  \hspace{-2mm} &
  \includegraphics[trim=0 0 0 0, clip, scale=.4750]{figures/ACM_TDS/partitioned/3-(b)-part.pdf}\\
  \small (a) 100 candidates & \small (b) 10,000 voters
  \end{tabular} 
   \vspace{-0.25cm}
  \caption{(a) Running time of the optimized algorithm and (b) speedup factor of the optimized algorithm over the baseline to compute the set of {\bf necessary winners} on \textbf{2-approval} scoring rule.}
  \label{fig:NW_2app}
\end{figure}
\begin{figure}%[b]
  \centering
  \begin{tabular}{c @{} c }
    % \includegraphics[width=.3333\linewidth]{example-image-a} &
    % \includegraphics[width=.3333\linewidth]{example-image-b} \\
    %\hspace{-3mm}\includegraphics[scale=.4750]{figures/ECAI/NW_Borda/(a)_m_final.pdf} \hspace{-2mm} & 
    %\includegraphics[scale=.4750]{figures/ECAI/NW_Borda/(a)_speedup_n_final.pdf}\\
    %\small (a) 100 candidates & \small (b) 10,000 voters\\
    \hspace{-3mm}\includegraphics[scale=.4750]{figures/ACM_TDS/partitioned/4-(a)-part.pdf} \hspace{-2mm} & 
    \includegraphics[scale=.4750]{figures/ACM_TDS/partitioned/4-(b)-part.pdf}\\
    \small (a) 100 candidates & \small (b) 10,000 voters
  \end{tabular}  
  %\caption{Running time of the optimized algorithm to compute the set of necessary winners,  100 candidates.}
   \vspace{-0.25cm}
  \caption{(a) Running time of the optimized algorithm and (b) speedup factor of the optimized algorithm over the baseline to compute the set of {\bf necessary winners} on \textbf{Borda} scoring rule.}
  \label{fig:NW_Borda}
\end{figure}

\subsection{Validation of RSM}\label{sec:exp:rsm}  

We conducted an experiment to verify that the Repeated Selection Model is sufficiently flexible to represent real partial voting profiles.  We extended the methods of Stoyanovich et al.~\cite{DBLP:conf/webdb/StoyanovichIP16} to fit a  RSM to the {\em dessert} dataset and to the {\em travel} dataset (both were described in Section~\ref{sec:poset:real}), observing the best fit with a RSM in both cases (Table~\ref{tab:nll}). 
\theo{Please note that we fit with one RSM, not a RSM Mix} 

{\colorThree 
More specifically, for each dataset, we compute the negative log-likelihood using the voters for whom we know both a full ranking $\rho$ and a partial ranking $T$:
\[
\mathcal{NLL} = -\frac{1}{n}\sum_{i}log(\mathbb{P}(T_i|\rho_i))
\]
Overall, RSM fits better to both the real world datasets when compared to the methods from Gehrlein's paper (lower negative log-likelihood values in Table~\ref{tab:nll} mean better fit \cite{DBLP:conf/webdb/StoyanovichIP16}).
% For the Dessert dataset, we isolate the voters for which we know both a full ranking $\rho$ and a partial ranking $T$ (around 110 voters) and we compute the negative log-likelihood:
% \[
% \mathcal{NLL} = -\frac{1}{n}\sum_{i}log(\mathbb{P}(T_i|\rho_i))
% \]
Synthetic methods fit the \emph{dessert} dataset better as compared to the \emph{travel} dataset because the latter contains partitioned preferences with missing candidates. The synthetic methods consider all the candidates appearing in its ranking for generating partial preferences making them a non-optimal fit to the \emph{travel} dataset. 
\begin{table}[]
    \centering
    \begin{tabular}{c|c|c|c}
    \toprule
        \multirow{2}{*}{\emph{Dataset}} & \multicolumn{3}{|c}{$\mathcal{NLL}$}  \\
        \cline{2-4}
         & \emph{Gehrlein 1} & \emph{Gehrlein 2} & \emph{RSM} \\
         \midrule\midrule
         \emph{Dessert (Sparse)} & $12.9$ & $14.7$ & $\mathbf{12.5}$\\ %\hline
         \midrule
         \emph{Dessert (Dense)} & $19.1$ & $19.8$& $\mathbf{18.7}$ \\ %\hline
         \midrule
         \emph{Travel} & $10.4$  &$10.4$ & $\mathbf{9.5}$\\ %\hline
    \bottomrule
    \end{tabular}
    \caption{Comparison of goodness-of-fit of synthetic data generation methods with real-world datasets. $\mathcal{NLL}$ stands for negative log-likelihood. Lower $\mathcal{NLL}$ value means better fit.}
    \label{tab:nll}
\end{table}
}


%We then quantified the correlations between the density distributions of the fitted models and those observed in the real datasets. We saw a very close fit, with Pearson's  $\rho = 0.89$ for the {\em travel} dataset, and $\rho = 0.96$ for {\em dessert}.

\subsection{Necessary Winners} 
\label{sec:exp:nw}

% \begin{figure*}[t!]
% \begin{subfigure}{.33\textwidth}
%   \centering
%   \includegraphics[width=0.975\linewidth]{figures/PW_m/PW-Borda-m=25_m_final.png}
%   \caption{\textbf{Borda}}
%   \label{fig:PW_m_Borda}
% \end{subfigure}%
% \begin{subfigure}{.33\textwidth}
%   \centering
%   \includegraphics[width=0.975\linewidth]{figures/PW_m/PW-Plurality-m=25_m_final.png}
%   \caption{\textbf{plurality}}
%   \label{fig:PW_m_plu}
% \end{subfigure}
% \begin{subfigure}{.33\textwidth}
%   \centering
%   \includegraphics[width=0.975\linewidth]{figures/PW_m/PW-2-approval-m=25_m_final.png}
%   \caption{\textbf{2-approval}}
%   \label{fig:PW_m_2app}
% \end{subfigure}
% \vspace{-0.1cm}
% \caption{Running time of the three-phase computation of the set of possible winners for 25 candidates.  6 out of 225 instances (2.7\%) timed out at 2,000 sec.  These were among only 37 instances that needed to execute the ILP solver in Phase 3.}
% \label{fig:PW_m}
% \end{figure*}


% \begin{figure*}[t]
% \begin{subfigure}{.33\textwidth}
%   \centering
%   \includegraphics[width=0.975\linewidth]{figures/PW_n/PW-Borda-n=10000_n_final.png}
%   \caption{\textbf{Borda}}
%   \label{fig:PW_n_Borda}
% \end{subfigure}%
% \begin{subfigure}{.33\textwidth}
%   \centering
%   \includegraphics[width=0.975\linewidth]{figures/PW_n/PW-Plurality-n=10000_n_final.png}
%   \caption{\textbf{plurality}}
%   \label{fig:PW_n_plu}
% \end{subfigure}
% \begin{subfigure}{.33\textwidth}
%   \centering
%   \includegraphics[width=0.975\linewidth]{figures/PW_n/PW-2-approval-n=10000_n_final.png}
%   \caption{\textbf{2-approval}}
%   \label{fig:PW_n_2app}
% \end{subfigure}
% %\vspace{-0.1cm}
% \caption{Running time of the three-phase computation of the set of possible winners for 10,000 voters.  4 out of 225 instances (1.8\%) timed out at 2,000 sec.  These were among only 24 instances that needed to execute the ILP solver in Phase 3.}
% %\vspace{-0.3cm}
% \label{fig:PW_n}
% \end{figure*}


We \st{now} first present experiments that demonstrate the impact of the  number of voters $n$ and the number of candidates $m$ on the running time of the optimized necessary winners algorithm described in Section~\ref{sec:nw}. In Figures~\ref{fig:NW_plurality}(a)-\ref{fig:NW_Borda}(a), we set $m=100$, vary $n$ between 10 and 10,000 on a logarithmic scale, and show the running time for each of the rules  plurality,  2-approval, and Borda, and for each family of synthetic datasets as a box-and-whiskers plot. We observe that the computation is efficient: %\rsmm
RSM Mix is the most challenging, and completes in 10 sec or less for 10,000 voters across all scoring rules. The running time increases linearly with $n$. 

Next, we \st{also}
analyzed  the \st{running time} \colorOne speed-up of optimized algorithm \colorTwo for $n=10,000$ voters, with $m$ ranging from $10$ to $200$ on a linear scale. Figures~\ref{fig:NW_plurality}(b)-\ref{fig:NW_Borda}(b) show these results in comparison to a baseline, where we reuse computation of $\textsc{Up}_{P}(c)$ and $\textsc{Down}_{P}(c)$  across candidates, but do not re-order candidates in a competition, and also do not optimize the computation of $\textsc{Up}_{P}(c)$ and  $\textsc{Down}_{P}(c)$  based on the structure of $P$.   The optimized implementation outperforms the baseline by a factor of 10-20 in most cases.  Overall, speed-up improves with increasing number of candidates, and  partial chain and \PWPV~datasets show the highest speed-up.  We see significant variability in Figure~\ref{fig:NW_plurality}(b), because some of the instances had  necessary winners and others did not.

We \colorOne also analyzed the running time and \colorTwo  observed that this computation is efficient: %\rsmm 
RSM Mix
completes in under 40 sec for $m=200$ for plurality and  2-approval, and for all except one case of Borda, where it takes 60 sec due to the presence of a necessary winner.  For  \PWPV~and partial chain, the computation completes in under 8.5 sec and 2 sec, respectively, pointing to the effectiveness of the optimizations that %compute $\textsc{Up}_{P}(c)$ and  $\textsc{Down}_{P}(c)$  based on 
use the structure of $P$.  


Finally, the running times were interactive on real datasets: 0.006 sec for all scoring rules on {\em dessert}, and 0.28 sec on {\em travel}. We achieved a factor of 2-2.5 speed-up over the baseline version for {\em dessert}, and a factor of 5 - 6.7 speed-up for {\em travel}.  Speed-up was most significant for Borda, with running time decreasing from 1.87 sec to 0.28 sec.

%Both tve thatmputation i thhis coe : {\e}s efficientsets of experiments are carried out across all types of datasets and all types of scoring rules. In the first experiment, we keep the number of candidates constant ($m$=100) and vary the number of voters (Figure \ref{fig:NW_m}), and in the second one, we keep the number of voters constant ($n$=10,000) and vary the number of candidates (Figure \ref{fig:NW_n}). As expected we saw a linear relationship between running time and number of voters across all datasets (Figure \ref{fig:NW_m}). Next, we saw running time increase exponentially with increase in candidates (Figure \ref{fig:NW_n}). Hence, we focus our analysis of speedup by keeping the number of voters constant. %Specifically for Figure 3, the outlier at 200 candidates for Borda was seen repeatedly across all experiments. The reason for that is there is a necessary winner (NW) in that particular dataset, leading to one of the instance of 200 candidates for Borda taking double the time as compared to when there is no NW. In the same plot, we see a similar trend for 150 candidates and Borda too; the reason is the same, presence of NW doubles the execution time of the optimized algorithm.

%Figure \ref{fig:NW_n_SU} presents the speedup of NW algorithm keeping number of voters constant. Overall, we saw that RSM had the least speedup among all datasets across all scoring rules due to the limited effect of optimizations on RSM dataset as discussed earlier in section ``Necessary Winners''. Further, we saw a couple of unexpected observations in our plots: (i) high variation in speedup of top-k dataset in Figure \ref{fig:NW_n_SU_2app} and (ii) running time of top-k dataset was higher for plurality as compared to Borda (Figures \ref{fig:NW_n_Borda} and \ref{fig:NW_n_plu}). A qualitative analysis led to an expected discovery that when $m$, $n$, dataset and scoring rule are the same, running time of optimized algorithm on instances without any NW was half the running time on instances with at least one NW. This is because we designed our optimizations, especially pruning ``necessary losers'', to work better when we have no NW, which is the case in most real world scenarios (e.g., we had no NW in dessert or travel datasets). Further, while we did see a significant drop in speedup in presence of a NW, there was no significant change due to the number of NW.

%\kunal{\emph{Real datasets}: There was no NW for either of the datasets across any of the scoring rules. Overall, we saw a speedup of 1.99, 2.57 and 2.06 for dessert data for borda, plurality and 2-approval respectively, and a speedup of 6.71, 5.05 and 5.10 for travel data respectively.}

%\begin{figure*}[t!]
%\begin{subfigure}{.33\textwidth}
%  \centering
%  \includegraphics[width=0.75\linewidth]{figures/NW_n/(a)_n.pdf}
%  \caption{\textbf{Borda}}
%  \label{fig:NW_n_Borda}
%\end{subfigure}%
%\begin{subfigure}{.33\textwidth}
%  \centering
%  \includegraphics[width=0.75\linewidth]{figures/NW_n/(b)_n.pdf}
%  \caption{\textbf{plurality}}
%  \label{fig:NW_n_plu}
%\end{subfigure}
%\begin{subfigure}{.33\textwidth}
%  \centering
%  \includegraphics[width=0.75\linewidth]{figures/NW_n/(c)_n.pdf}
%  \caption{\textbf{2-approval}}
%  \label{fig:NW_n_2app}
%\end{subfigure}
%\caption{The running time of the optimized necessary winner algorithm.  The number of voters is fixed at $10,000$.}
%\label{fig:NW_n}
%\end{figure*}

\subsection{Possible Winners}
\label{sec:exp:pw}

\begin{figure}[t]
  \centering
  \begin{tabular}{c @{} c }
  %\hspace{-3mm}\includegraphics[scale=.475]{figures/ECAI/PW_Plu/(b)_PW_plu_m.pdf} \hspace{-2mm} &
  %\includegraphics[trim=0 0 0 0, clip, scale=.4750]{figures/ECAI/PW_Plu/(b)_PW_plu_n.pdf}\\
  %\small (a) 25 candidates & \small (b) 10,000 voters\\
  \hspace{-3mm}\includegraphics[scale=.475]{figures/ACM_TDS/partitioned/5-(a)-part.pdf} \hspace{-2mm} &
  \includegraphics[trim=0 0 0 0, clip, scale=.4750]{figures/ACM_TDS/partitioned/5-(b)-part.pdf}\\
  \small (a) 25 candidates & \small (b) 10,000 voters
  \end{tabular} 
  \vspace{-0.25cm}
  \caption{Running time of the computation of the set of {\bf possible winners} on \textbf{plurality},  using optimized algorithm from Betzler and Dorn \cite{DBLP:journals/jcss/BetzlerD10}.
  }
  \label{fig:PW_Plurality}
\end{figure}

Figure~\ref{fig:PW_Plurality} shows the running time of the computation of the set of possible winners on plurality, using the algorithm from Betzler and Dorn \cite{DBLP:journals/jcss/BetzlerD10}, with our optimizations (see Section~\ref{sec:pw-betzler-dorn}).  In Figure~\ref{fig:PW_Plurality}(a), we set $m=25$ and vary $n$ between 10 and 10,000 on a logarithmic scale, while in Figure~\ref{fig:PW_Plurality}(b) we set $n=10,000$ and vary $m$ between 5 and 25 on a linear scale.  We observe that this algorithm is efficient: most instances complete in less than 0.5 sec, with the exception of a single instance that takes just over 1 sec. The running time is higher when there are more {\colorOne number of} possible winners.  For this reason, computation is fastest on \PWPV~datasets, and slowest on partial chain datasets.  (Note that we set $m$ lower {\colorOne for possible winner experimentals} than for necessary winners, where $m$ went up to 200, to have the same experimental setting as for 2-approval and Borda, discussed later in this section.  A high value of $m$ is infeasible for these rules, because of the intrinsic complexity of computation.)

%\kunal{need to add discussion on Figure~\ref{fig:PW_Plurality}, poly-time algorithm for PW and plurality. To this end, important observations for Figure~\ref{fig:PW_Plurality}(a): (i) All instances of all datasets compute the set of PW in less than 0.5 sec except 10,000 voters and linear which take just over 1 sec. (ii) The time taken by each dataset is directly proportional to the number of candidates who are possible winners (all candidates in linear dataset are always possible winners, hence it is the slowest. Similarly, top-k has the lowest number of PW, hence the fastest.) Important observations for Figure~\ref{fig:PW_Plurality}(b): (i) Trend across datasets is for the same reason as discussed for Figure~\ref{fig:PW_Plurality}(a) (all instances, except linear and 10,000 voters, take less than 0.3 sec, and the time taken is directly proportional to the number of PWs). (ii) The reason for sudden rise in instances of linear dataset with 25 candidates is unknown (we can possibly attribute it to the fact that small variability (rise in running time by 0.8 sec) in instances with low running times (around 0.3 sec) can seem massive (though this reason doesn't seem justifiable)).}

%\balance 

Next, we \st{now} present experiments \kunal{We use `experimentals' and `experiments' interchangeably. It may be helpful to remain consistent with terminology.} that demonstrate the impact of the  number of voters $n$ and the number of candidates $m$ on the running time of the three-phase computation described in Section~\ref{sec:possible:threephase}. \st{As for necessary winners,} We fix $m$ at 25 and vary $n$ between 10 and 10,000 on a logarithmic scale, and then fix $n$ at 10,000 and vary $m$ between 5 and 25 on the linear scale. % Because of the intrinsic complexity of the problem, we vary $m$ between 5 and 25.  (This is in contrast to necessary winners, where $m=200$ was feasible.) 
%
Even with these modest values of $m$, the ILP solver can take a very long time.  Thus, to make our experimental evaluation manageable, we set an end-to-end cut-off of 2,000 sec per instance.  In what follows, we report the running times of the instances that completed within the cut-off, and additionally report the percentage of completed instances.


%\kunal{Statistics for 2-approval (I think merging the numbers for 2-approval and Borda is a better idea): (A) for number of voters on x-axis (Figure~\ref{fig:PW_2app}(a)): Among the 75 instances we executed for this experiment, only 13 (17.3\%) needed to execute Phase 3 (the ILP solver) with 3 or fewer candidates to check, and none of these timed out at 2,000 sec. Instances that didn't need Phase 3 (ILP solver) computed the set of possible winners in under 55 sec (median 0.93 sec, mean 9.20 sec, stdev 15.96 sec). In contrast, instances that needed Phase 3 computed the set of possible winners in under 148 sec (median 8.46 sec, mean 30.69 sec, stdev 48.72 sec). (B) for number of candidates on x-axis (Figure~\ref{fig:PW_2app}(a)): Among the 75 instances we executed for this experiment, only 9 (12.0\%) needed to execute Phase 3 (the ILP solver) with 2 or fewer candidates to check, and none of these timed out at 2,000 sec. Instances that didn't need Phase 3 (ILP solver) computed the set of possible winners in under 55 sec (median 2.42 sec, mean 10.88 sec, stdev 15.02 sec). In contrast, instances that needed Phase 3 computed the set of possible winners in under 148 sec (median 96.80.46 sec, mean 83.36 sec, stdev 38.25 sec).}

Figures~\ref{fig:PW_2app}(a) and \ref{fig:PW_Borda}(a) show the running time as a function of the number of voters for 2-approval and Borda, respectively. The running time increases linearly with the number of voters.  Interestingly,  partial chain datasets take as long or longer to process as %\rsmm 
RSM Mix datasets.  This is because Phase 1 is more effective for % \rsmm
RSM Mix, with fewer candidates passed on to Phase 2.

Phases 1 and 2 are effective in pruning non-winners and in identifying clear possible winners. Of the 75 instances we executed for this experiment for each scoring rule, only 13 (17\%) needed to execute Phase 3 (i.e., invoke the ILP solver) for 2-approval, and only 9 (12\%) ---  for Borda, with at most 3 candidates to check. % Of these, 26  had one candidate to check, 8 had two candidates, and 3 had three candidates.  
Of the 9 instances that reached Phase 3 for Borda, 6 timed out at 2,000 sec.  No other instances timed out in this experiment.  Instances reaching Phase 3 are responsible for the high variability in the running times. For 2-approval, all instances that reached Phase 3 computed in under 148 sec (median 8.46 sec, mean 30.69 sec, stdev 48.72 sec). \kunal{As done for Borda later in this paragraph, do we want to add statistics for 2-approval for instances that that did not execute Phase 3? (max=55 sec, median 0.96 sec, mean 9.38 sec, stdev 16.01 sec))} For Borda, for the three instances that executed Phase 3 and did not timeout, the running times were 6 sec, 15 sec, and 381 sec.  In contrast, all remaining instances --- those that did not execute Phase 3 --- computed in under 53 sec (median 2.44 sec, mean 9.50 sec, stdev 15.14 sec).
%In contrast, all remaining instances --- those that did not execute Phase 3 --- computed in under 55 sec (median 2.42 sec, mean 10.88 sec, stdev 15.02 sec) for \emph{2-approval}, and in under 53 sec (median 2.11 sec, mean 9.01 sec, stdev 14.76 sec) for \emph{Borda}. 

Figures~\ref{fig:PW_2app}(b) and~\ref{fig:PW_Borda}(b) show the running times as a function of the number of candidates under 2-approval and Borda.  We make similar observations here as in our discussion of Figures~\ref{fig:PW_2app}(a) and~\ref{fig:PW_Borda}(a), noting that only 9 instances instances reached Phase 3 for 2-approval, and only 4 reached Phase 3 for Borda.  These instances {\colorOne, all RSM Mix,} took longer to run, and contributed the most to running time variability.

\colorThree
We now compare the running times of the three-phase computation described in Section~\ref{sec:possible:threephase} with a polynomial-time algorithm for 2-approval and partitioned preferences \cite{DBLP:conf/atal/Kenig19}. Figure~\ref{fig:PW_2app}(c) shows the running times as a function of the number of partitions for instances containing 25 candidates and 10,000 voters. None of the 30 instances needed ILP (Phase 3) while using the three-phase computation. Overall, our approach, which is more generalized as it works for \emph{all} the variations of the PW problem, is faster than the polynomial-time algorithm when Phase 3 is not needed. 
\colorTwo

%among the 75 instances we executed for this experiment on \emph{Borda}, only 4 (5.3\%) needed to execute Phase 3 (the ILP solver) with 2 or fewer candidates to check, and all 4 of these timed out at 2,000 sec. 
%All instances that did not execute Phase 3 computed the set of possible winners in under 53 sec (median 6.85 sec, mean 12.54 sec, stdev 13.92 sec).  

%Results for \emph{2-approval} are shown in Figure~\ref{fig:PW_2app}(b), with Phase 3 invoked for 9 instances, all of which computed in under 148 sec (median 96.81 sec, mean 83.36 sec, stdev 38.25 sec).  Instances that did not execute Phase 3 computed in under 55 sec (median 2.42 sec, mean 10.88 sec, stdev 15.02 sec).
%julia{Kunal, please add the numbers, I'll make another pass tomorrow morning.  I don't have any time left this evening.}
%We evaluated the efficacy of the three-step candidate pruner and measured the new running times. Figure \ref{fig:PW_m} and Figure \ref{fig:PW_n} show the running time of the optimized algorithm. We observed that the overall running time is significantly lower than the ILP implementation using Gurobi, and more importantly, only 10\% of instances reach the cut-off time of 2000 seconds. Thus, we also analyzed the number of candidates getting pruned after each step. Overall, we saw that the instances that needed Gurobi (3$^{rd}$-step) were much slower and hence, usually reached the cut-off time.   

%We first analyze the anomalies in the running time of instances. Figure \ref{fig:PW_m} has a high variance for RSM across all 3 scoring rules, especially for Borda, owing to the need to call Gurobi on multiple instances. Next, Figure \ref{fig:PW_n_Borda} also has a high variation as one of the instances has a PW which needs Gurobi implementation, and that too it needs Gurobi for a very long time. 

%Next, we analyze the number of candidates that get pruned during each step. Step 1 pruning is the most efficient for top-k dataset (specifically, 2-approval and plurality). Step 2 pruning, specifically for 2-approval and Borda scoring rule, and for drop candidate dataset, is very efficient with almost 90\% of the candidates getting pruned during this step. The use of Up/Down from Xia and Conitzer while building completions to find PW is efficient on drop candidate dataset due to its linearity, which makes it easier to find a possible world where a candidate is a winner. Except for one instance when Gurobi (step 3) is needed for drop candidate dataset (m=25, n=10, 2-approval and drop-candidate), it is otherwise always needed by RSM dataset. This anomaly can be attributed to lesser number of candidates being pruned in that particular instance of the drop candidate dataset which makes it difficult to build completions in step 2. Overall, we saw that the time needed to build completions has low variance across different experiments, but the time needed to solve using Gurobi varies a lot. Further, the speedup is expectantly higher when we only need the first two steps. Finally, based on our analysis of the number of candidates reaching the Gurobi step, we found no correlation (Pearson's $\rho<0.30$, p$<$0.05, $\alpha$=0.05) between the number of candidates that need Gurobi (step 3) and the time taken by Gurobi. We validated this qualitatively for RSM dataset, Borda scoring rule, $m$=20 and $n$=100, where an instance which needs Gurobi for 10 candidates is around 10 times faster than an instance which needs Gurobi for 6 candidates.
\begin{figure}[t]
  \centering
  \begin{tabular}{c @{} c @{} c }
  %\hspace{-3mm}\includegraphics[scale=.475]{figures/ECAI/PW_2app/PW-2-approval-m=25_m_final.pdf} \hspace{-2mm} &
  %\includegraphics[trim=0 0 0 0, clip, scale=.4750]{figures/ECAI/PW_2app/PW-2-approval-n=10000_n_final.pdf}\\
  %\small (a) 25 candidates & \small (b) 10,000 voters\\
  \hspace{-3mm}\includegraphics[scale=.475]{figures/ACM_TDS/partitioned/6-(a)-part.pdf} \hspace{-2mm} &
  \includegraphics[trim=0 0 0 0, clip, scale=.4750]{figures/ACM_TDS/partitioned/6-(b)-part.pdf}&
  \includegraphics[trim=0 0 0 0, clip, scale=.4750]{figures/ACM_TDS/partitioned/6-(c)-part.pdf}\\
  \small (a) 25 candidates & \small (b) 10,000 voters & \small (c) 25 candidates \& 10,000 voters
  \end{tabular} 
  \vspace{-0.25cm}
  \caption{Running time of the three-phase computation of the set of {\bf possible winners} on \textbf{2-approval} scoring rule. (a) None of the 75 instances timed out at 2,000 sec.  These were among only 13 instances (9 RSM Mix and 4 partial chain) that needed to execute the ILP solver in Phase 3. (b) None of the 75 instances timed out at 2,000 sec. These were among only 9 instances (all RSM Mix) that needed to execute the ILP solver in Phase 3. (c) Comparison of three-phase computation with polynomial-time algorithm (based on flow network and theoretical results in \cite{DBLP:conf/atal/Kenig19}) by varying the number of partitions in each instance.
  }
  \label{fig:PW_2app}
\end{figure}

\begin{figure}[t]
  \centering
  \begin{tabular}{c @{} c}
  %\hspace{-3mm}\includegraphics[scale=.475]{figures/ECAI/PW_Borda/PW-Borda-m=25_m_final.pdf} \hspace{-2mm} &
  %\includegraphics[trim=0 0 0 0, clip, scale=.4750]{figures/ECAI/PW_Borda/PW-Borda-n=10000_n_final.pdf}\\
  %\small (a) 25 candidates & \small (b) 10,000 voters\\
  \hspace{-3mm}\includegraphics[scale=.475]{figures/ACM_TDS/partitioned/7-(a)-part.pdf} \hspace{-2mm} &
  \includegraphics[trim=0 0 0 0, clip, scale=.4750]{figures/ACM_TDS/partitioned/7-(b)-part.pdf}\\
  \small (a) 25 candidates & \small (b) 10,000 voters
  %\hspace{-3mm}\includegraphics[scale=.475]{figures/ACM_TDS/partitioned/7-(a)-botk.pdf} \hspace{-2mm} &
  %\includegraphics[trim=0 0 0 0, clip, scale=.4750]{figures/ACM_TDS/partitioned/7-(b)-botk.pdf}\\
  %\small (e) 25 candidates & \small (f) 10,000 voters
  \end{tabular} 
  \vspace{-0.25cm}
  \caption{Running time of the three-phase computation of the set of {\bf possible winners} on \textbf{Borda} scoring rule. (a) 6 (all RSM Mix) out of 75 instances (8.0\%) timed out at 2,000 sec.  These were among only 9 instances (all RSM Mix) that needed to execute the ILP solver in Phase 3. (b) 4 (all RSM Mix) out of 75 instances (5.3\%) that needed to execute the ILP solver, timed out at 2,000 sec.
  }
  \label{fig:PW_Borda}
\end{figure}
{\colorThree

Next, we measured the efficiency of the first two phases of the three-phase computation, which do not require an ILP-solver and is polynomial in the size of candidates, by calculating the proportion of profiles for which the three-phase computation terminates after the first two phases. We created 10,000 profiles consisting of 100 voters and 10 candidates using a mixture of three RSMs. The parameters were chosen uniformly at random.
%we computed the set of possible winners using different generalized poset generation methods (Method 1, Method 2 \cite{gehrlein1986methods}, and RSM).  
Our pruning mechanism was able to find the entire set of possible winners for 91.62\% of profiles after the first two phases, thus not needing an ILP-solver (Figure~\ref{fig:RSM_sucess_dataset}).
%for which parameters and which density we obtain "hard" profiles with RSM, i.e. profiles for which the first two phases of the PW algorithm cannot conclude for all the candidates, and we need to use the ILP solver for at least one of them. In this experiments, we use 10,000 profiles of 100 voters and 10 candidates, with a mixture of three RSM and parameters taken at random. 
Furthermore, the first two phases failed mostly when the $\phi$ parameter was low and the average density was medium, or when the $\phi$ parameter as well as the average density were both high. Profiles with low average density always terminated after the second phase. 

We also compared the average running time of the first two phases of the PW algorithm using RSM profiles with profiles generated using Gehrlein's methods. RSM profiles generally take more time across different values of phi (Figure~\ref{fig:running_time_success}(a)) and across different poset densities (Figure~\ref{fig:running_time_success}(b)) as RSM is more generalized  (Figure~\ref{fig:RSM_eval_gehrlein}).
%Figure~\ref{fig:running_time_success} also shows that the running time depends a lot on the Mallows parameter $\phi$ and the density of the profile.
}


Finally, {\colorOne as our three-phase computation was found to be more efficient,} we computed the set of possible winners for the real datasets {\em dessert} and {\em travel} {\colorOne using our approach}, and found multiple possible winners for all scoring rules.  In all cases, winners were determined in Phases 1 and 2 of the three-phase computation (Section~\ref{sec:possible:threephase}). %, and Phase 3 was not required.  
All executions completed within at most 22.47 sec.  \st{For example,}{\colorOne More importantly,} the set of possible winners under Borda for {\em dessert} took 1.39 sec to compute with three-phase computation, and 2.37 sec when each candidate was considered with only the two-phase \st{computation} {\colorOne subroutine} (i.e., invoking repeatedly the ILP solver as in Section~\ref{sec:possible:ilp}).  More dramatically, three-phase computation under {\em Borda} took 22.47 sec on  {\em travel}, and did not complete within  2,000 sec using only the two-phase \st{computation} {\colorOne subroutine}.
\kunal{Alternate write-up: ``... at most 22.47 sec. More importantly, computing the set of possible winners under Borda for {\em dessert} using three-phase computation was faster than  using only the two-phase subroutine (i.e., invoking the ILP solver for each candidate - Section~\ref{sec:possible:ilp}) (1.39 sec vs 2.37 sec). More dramatically, ....''}
{\colorOne}

\colorOne

%\subsection{Partitioned Preferences and its variants}
%\kunal{this subsection (6.3) should be removed.}
%We also conducted two sets of experiments to specifically analyze the difference in running time between \PWPV, \PWDV, \PWTV, and \PWBV  when using $m=25$ candidates, $n=10,000$ voters and 2-approval scoring rule.

%\subsubsection{Constant number of partitions}
% In the first experiment, we restricted the number of partitions $p$ (see \ref{sec:partionedpref} for formal definition) for all the four types of partial orders. Further, all experiments reported were carried out on 5 different datasets to account for any outliers.
 
% The time taken to compute the set of possible winners decreases as the value of $p$ (or the number of partitions) increases (Figure~\ref{fig:partitionTest}). Also, top-truncated dataset was the fastest as we terminate the algorithm as soon as we find a possible world where a candidate wins. Similarly, we conducted experiments for finding the set of necessary winners as well and found that bottom-truncated dataset was the fastest for NW problem as we terminate the algorithm as soon as we find a possible world where a candidate loses.
 
%\subsubsection{Varying number of partitions}
%In the second experiment, we chose the number of partitions $p$ for each voter uniformly at random and otherwise kept all the parameters same as the previous section. Overall, we observed the top-truncated dataset to be the fastest for PW problem and bottom-truncated dataset for the NW.

\colorTwo

\begin{figure}[t]
    \centering
    %\includegraphics[scale=0.475]{figures/ACM_TDS/RSM/RSM_HardnessTime_TDSphi.pdf}
    %\includegraphics[scale=0.475]{figures/ACM_TDS/RSM/RSM_HardnessTime_TDSdensity.pdf}
    %\includegraphics[scale=0.475]{figures/ACM_TDS/RSM/RSM_Hardness_TDS_v2.pdf}
    \includegraphics[scale=0.475]{figures/ACM_TDS/RSM/RSM_Hardness_TDS.pdf}
    
\vspace{-0.5cm}
  \caption{\colorThree 91.62\% of 10,000 RSM profiles, each consisting of 10 candidates and 100 voters, found the entire set of possible winners after the first two phases of pruning without the need of using ILP (Gurobi). \kunal{Julia, let us move figure 6(c) here as 8(a)? Overall, this figure will contain 2 plots, which will be referred to when we discuss effectiveness/efficiency of three-phase computation.}
  }
 % \vspace{-0.3cm}
  \label{fig:RSM_sucess_dataset}
\end{figure}

\begin{figure}[t]
  \centering
  \begin{tabular}{c @{} c }
  \hspace{-3mm}\includegraphics[scale=.475]{figures/ACM_TDS/RSM/RSM_HardnessTime_TDSphi.pdf} \hspace{-2mm} &
  \includegraphics[trim=0 0 0 0, clip, scale=.4750]{figures/ACM_TDS/RSM/RSM_HardnessTime_TDSdensity.pdf}\\
   \small (a) & \small (b) 
  \end{tabular} 
  \vspace{-0.25cm}
  \caption{ \colorThree Average running times of the first two phases of the three-phase computation for successful cases using Borda scoring rule (Method 1 and Method 2 are from Gehrlein~\cite{gehrlein1986methods}).}
  \label{fig:running_time_success}
\end{figure}

\begin{figure}[t]
    \centering
    %\includegraphics[scale=0.475]{figures/ACM_TDS/RSM/RSM_HardnessTime_TDSphi.pdf}
    %\includegraphics[scale=0.475]{figures/ACM_TDS/RSM/RSM_HardnessTime_TDSdensity.pdf}
    %\includegraphics[scale=0.475]{figures/ACM_TDS/ExpSetup1-PW.png}
    %\includegraphics[scale=0.1]{figures/1.pdf}
    %\includegraphics[scale=0.1]{figures/2.pdf}
    %\includegraphics[scale=0.1]{figures/RSM_example/RSM_example.pdf}
    \includegraphics[trim=400 0 0 0, clip,scale=0.12]{figures/RSM_example/RSM_example_v6.pdf}
    %\includegraphics[trim=400 0 0 0, clip,scale=0.12]{figures/RSM_example/RSM_example_v7.pdf}
    
\vspace{0cm}
  %\caption{\colorThree Computing the set of possible winners using polynomial-time algorithm on 25 candidates, 10,000 voters, and 2-approval scoring rule. (top: top-truncated, bottom: bottom-truncated, doubly:doubly-truncated) \kunal{Remove the figure and also move the discussion.}}
  \caption{Example 1 of 2: A stepwise representation of the RSM method. \kunal{caption is incomplete.}}
 % \vspace{-0.3cm}
  \label{fig:RSM_example1}
\end{figure}

\begin{figure}[t]
  \centering
  \begin{tabular}{c}
  %\hspace{-3mm}\includegraphics[scale=.475]{figures/ECAI/PW_Borda/PW-Borda-m=25_m_final.pdf} \hspace{-2mm} &
  %\includegraphics[trim=0 0 0 0, clip, scale=.4750]{figures/ECAI/PW_Borda/PW-Borda-n=10000_n_final.pdf}\\
  %\small (a) 25 candidates & \small (b) 10,000 voters\\
  \hspace{-3mm}\includegraphics[trim=215 0 0 0, clip,scale=0.11]{figures/RSM_example/RSM_example_comb_v1_p1.pdf}\\
  \small (a) \\
  \includegraphics[trim=215 0 0 0, clip,scale=0.11]{figures/RSM_example/RSM_example_comb_v2_p2.pdf}\\
   \small (b) \\
  %\includegraphics[trim=0 0 0 0, clip, scale=.4750]{figures/ACM_TDS/partitioned/7-(b)-part.pdf}\\
  %\small (a) 25 candidates & \small (b) 10,000 voters
  %\hspace{-3mm}\includegraphics[scale=.475]{figures/ACM_TDS/partitioned/7-(a)-botk.pdf} \hspace{-2mm} &
  %\includegraphics[trim=0 0 0 0, clip, scale=.4750]{figures/ACM_TDS/partitioned/7-(b)-botk.pdf}\\
  %\small (e) 25 candidates & \small (f) 10,000 voters
  \end{tabular} 
  \vspace{-0.25cm}
  \caption{Example 2 of 2: A stepwise representation of the RSM method. \kunal{caption is incomplete.}}
  \label{fig:RSM_example2}
\end{figure}

%\kunal{Result from implementing poly-time algorithm for PW and plurality on real datasets: dessert takes 0.005 sec (vs 0.353 sec when using 3-phase computation) and travel takes 0.790 sec (vs 0.526 sec when using 3-phase computation). }

%\kunal{\emph{Real datasets:} We get multiple PWs for each dataset across all the scoring rules as expected. Further, all the candidates were pruned in the first two steps, and hence, Gurobi wasn't needed for any of the datasets using any of the scoring rule. In other words, we had a 100\% pruning rate, which overall took up to 3.11 seconds.}

%\theo{
%(i) For Plurality, the optimization are not really reducing the running time (speedup of 2 in average). But it is not a problem because for this rule we already have an algorithm which is 500 times faster. (ii) For 2-approval, we can see the effect of the optimization, but it is not a huge speedup, around 3 times faster in average. It is due to the fact that gurobi for k approval is actually pretty fast. (iii) For Borda, the optimized algorithm is really faster than the ILP only. For instance, it is in average 1961 times faster for RSM, Borda, m=25, n= 100, and this number increase with m and n. (iv) we notice that time to build a completion does not vary a lot throught the different experiments, but the time to solve an ILP vary a lot. (v) Obviously, the speedup is higher when we only need the first two steps.
%}

%\vishal{Step 2 has two parameter settings. For the experiments run by Theo, these are 2 and 3 which act as "cut-offs". The difference between time taken by Step 2 when it converges for a candidate before the cut-off, and when it does not, is in milliseconds. There is a variation, however it is not noticeable. The time taken by Step 2 for a (m,n) will hardly vary in a dataset for a given rule.}

==> tex_files/ack.tex <==
\begin{acks}
\end{acks}



==> tex_files/cover.tex <==
Dear Editor,

It is our pleasure to submit for your consideration our paper on algorithmic techniques for determining the necessary and possible winners in an election.  In this work we investigate the practical aspects of these important and intellectually exciting problems from Computational Social Choice (COMSOC), where they have so far received primarily theoretical treatment.  We bring an important insight from the point of view of the data management community, namely, that it is crucial to show practical applicability of techniques using a combination of real datasets and synthetic benchmarks.  The benchmark we propose here - the Repeated Selection Model - is a novel generative model for posets.  It gives the flexibility to us, and others, to systematically evaluate performance of winner determination methods in a wide range of scenarios.

Sincerely,
.....

==> tex_files/poset.tex <==
\section{Poset Generation}

In this section we describe a novel generative model for posets called the Repeated Selection Model, or RSM for short.  This model is of independent interest, and we use it here as part of our experimental, described in Section~\ref{sec:exp}.

\subsection{Synthetic Datasets}\label{sec:poset:synth}
We used three different types of synthetic datasets, which we call \emph{Partial chain}, \emph{\st{Top-$k$} partitioned} , and \rsmm.  
The  datasets of the first two types were obtained via the \emph{Mallows model}, which is a well known generative model for total orders~\cite{Mallows1957}; the datasets of the third type were obtained via the
\emph{Repeated Selection Model} (RSM), which is a new generative model for partial orders that we introduce in this paper. 

\subsubsection{Partial chains and partitioned preferences}

A \emph{Mallows model} over a set $A$ of $m$ items specifies a generator of a random total order on $A$ using two parameters: a \emph{reference ranking} $\sigma$, which is a total order on $A$, and a \emph{dispersion parameter} $\phi$, which is a number in the interval $[0,1]$. Such a model
defines a probability space over the  permutations on $A$, where the probability of a permutation $\rho$ is defined as follows:
\begin{align}
  \mathrm{Pr}(\rho|\sigma,\phi) =
  \frac{\phi^{d_{\textsc{kt}}(\sigma,\rho)}}{\sum_{\rho'}
    \phi^{d_{\textsc{kt}}(\sigma,\rho')}}.
\end{align}
Here,  $d_{\textsc{kt}}$ is the \emph{Kendall-Tau distance} defined as the number of inversion between the two rankings :
\begin{align*}
    d_{\textsc{kt}}(\sigma,\rho) =
    |\{(i,j) : (i >_{\sigma} j \wedge i <_{\rho} j) \}|.
\end{align*}
%\theo{I changed the above definition of Kandall-Tau distance with a much simpler equivalent definition.}
In particular, $\phi = 1$ gives the uniform distribution over the set
of all possible permutations; furthermore, the closer $\phi$ is to zero, the
more concentrated the distribution is around $\sigma$.  


%\begin{itemize}
%    \item 
\paragraph{Partial chains} A \emph{partial chain} on a set $A$ of $m$ items is a total order on a subset $B$ of $A$.

Our partial chain datasets are generated via Mallows models as follows.
Start with a total voting profile ${\bf T}=(T_1,\ldots,T_n)$, drawn from a mixture of three Mallows, each with $\phi=0.5$,  with a randomly chosen $\sigma$ of size $m$, and covering approximately $\frac{1}{3}$ of the voters.  For each $T_i$, choose $d \in [0,m-2]$ uniformly at random.  Drop $d$ candidates from $T_i$ by selecting one uniformly at random from the remaining candidates over $d$ iterations.  Return $P_i$ as a partial chain partial order.
    


{\colorOne    
\paragraph{Partitioned preferences}\label{sec:partionedpref}
By definition, a \emph{partitioned preference partial order} on a set $A$ of $m$ items is a total order over multiple subsets of unordered items from set $A$ (i.e., each subset contains items with no relative preferences among them). For example, in a rating system similar to the \emph{travel} dataset, each user rates items using an integer number between one and five. In such cases, we can not order items having a same rating, but we can have a total order of such subsets of items. 

%Partitioned preferences provide a good compromise between complete orders and arbitrary partial orders. Intuitively, the user pro- vides a complete order over sets of incomparable items. In the machine learning community, partitioned preferences were shown to be common in many real-life datasets, and have been used for learning statistical models on full and partial rankings [10, 13, 14]. In recommender systems, the items are often partitioned according to their numerical level of desirability [16] (e.g., the common star- rating system, where the scores range between 1 and 5 stars). In such a scenario, all items with identical scores are incomparable. Partitioned profiles are also used to represent agent preferences in resource allocation problems [1].


Previous work \cite{DBLP:conf/atal/Kenig19,dey2016exact,baumeister2012campaigns} has discussed several restrictions of partitioned preferences, namely top-truncated, bottom-truncated, and doubly-truncated. 
%\emph{Top-truncated} partial orders contain linear order on the top, followed by totally unordererd set, \emph{bottom-truncated} partial orders contain totally unordererd set on the top, followed by linear order at bottom, and \emph{doubly-truncated} partial orders contain linear order on top, followed by totally unordererd set, followed by linear order at bottom. 
We empirically analyzed the running time of calculating a set of possible winners using polynomial time algorithm for these restrictions of partitioned preferences using plurality and $k$-approval scoring rules, and didn't see any significant difference in the rate of change of running time between these restrictions of partitioned preferences across each scoring rule (Student’s t-test, p >0.05). No significant difference was seen for computing a set of necessary winners across these datasets using plurality, $k$-approval and Borda scoring rules as well. Hence, we used partitioned preferences for our experiments as they are more generalized:

%Our partitioned preference dataset is generated by s
Start with a total voting profile ${\bf T}=(T_1,\ldots,T_n)$, drawn from a mixture of three Mallows as for {\em partial chain}. 
For each $T_i$, choose $p \in [2,m]$, number of subsets $T_i$ will be partitioned into, uniformly at random, and split the total order $T_i$ into $p$ subsets. 
Next, select $p-1$ positions between 2 and $m$ uniformly at random without replacement such that the subsets will be partitioned at these positions. Drop the order relations among the candidates within each subset.
%for each subset $i \in [1,p]$, starting from the first one, assign a number of candidates, selected from the range $[1,(m-r)-(p-i)]$ uniformly at random, to the subset $i$ ($r$ = number of candidates previously assigned to some subset), and drop the order relations among the candidates within the subset $i$. The last subset gets all the remainder of the candidates.

}    

\paragraph{Top-truncated}
\julia{special case of partitioned, may drop from here or mention briefly; also mention bottom-truncated and doubly-truncated if we keep these}
By definition, a \emph{top-$k$} partial order on a set $A$
of $m$ items, where $k\leq m$, is a partial order 
consisting of a linear order of the highest-ranked $k$ items, followed by $m-k$ unordered items (i.e., $m-k$ items with no relative preferences among them).
   
Our top-$k$ datasets are generated via Mallows models as follows.   
    Start with a total voting profile ${\bf T}=(T_1,\ldots,T_n)$, drawn from a mixture of three Mallows as for {\em partial chain}. For each $T_i$, choose $k \in [1,m-1]$ uniformly at random.  Return a linear order of the highest-ranked $k$ items, followed by $m-k$ unordered items.


    \subsubsection{Complexity of Possible Winners on partial chain and Top-k} \label{section:pw-k}
    \kunal{This subsection needs to go. The complexity results are now discussed in section~\ref{sec:preliminaries}.}
    Both partial chains and top-k partial orders are collections of partial orders obeying certain structural restrictions.  Thus, it is  natural to ask whether the NP-hardness results for possible winners given in  Theorem \ref{class-thm} (Classification Theorem)  still hold true when the input partial profiles are restricted to be partial chain or are restricted to be top-k.
 
    As regards partial chain profiles, we are able to establish NP-hardness for some of the main positional scoring rules.
    
    \begin{theorem} \label{linear-thm} If $r$ is the Borda rule or the $t$-approval rule with $t\geq 4$, then the following problem is NP-complete: given a partial chain profile {\bf P} and a candidate $c$, is $c$ a possible winner w.r.t.\ $r$ and {\bf P}?
    \end{theorem}
    The proof of Theorem \ref{linear-thm} involves non-trivial reductions that use, among other things, constructions of auxiliary total profiles with special properties that appeared earlier  in \cite{dey2016exact,DBLP:journals/jair/XiaC11}. 
    %\kunal{Do we need to include a proof of this reduction?}
    
    It is an open problem whether computing possible winners remains NP-hard for $2$-approval and for $3$-approval, when the input partial profiles are partial chain.
    
    As regards top-k partial profiles, the following results have been established earlier in \cite{betzler2011unweighted,davies2011complexity} for the Borda rule, and in \cite{baumeister2012campaigns} for the $t$-approval rule,  for each $t\geq 2$.
    
    \begin{theorem} \label{top-k-thm} The following statements are true.
    \begin{itemize}
        \item \emph{ \cite{betzler2011unweighted,davies2011complexity}} If $r$ is the Borda rule, then the following problem is NP-complete: given a top-$k$ partial profile {\bf P} and a candidate $c$, is $c$ a possible winner w.r.t.\ $r$ and {\bf P}?
        \item \emph{\cite{baumeister2012campaigns}} If $r$ is the $t$-approval rule, where $t\geq 2$, then the following problem is solvable in polynomial time: given a top-$k$ partial profile {\bf P} and a candidate $c$, is $c$ a possible winner w.r.t.\ $r$ and {\bf P}?
    \end{itemize}
    \end{theorem}
    
     Theorems \ref{linear-thm} and \ref{top-k-thm} tell us  that computing possible winners under the Borda rule remains an NP-hard problem even when the partial profiles are restricted to be partial chain or restricted to be top-$k$.
     
    %\kunal{Need to add optimizations done to Baumeister’s and Kenig's algorithms used for computing the set of PW using $t$-approval  and partitioned preferences (top-$k$); also optimizations done to plurality algorithm.}
    
    \subsubsection{Repeated Selection Model (RSM) and RSM Mix}
    
   {\colorThree
    Existing partial order generation methods follow two independent steps: \begin{enumerate}
        \item Sample a complete ranking $\rho$ from some probabilistic model (see Marden~\cite{marden}).
        \item Sample a partial order from the full ranking $\rho$ by selecting only a subset of all the preference pairs.
    \end{enumerate}
    }
    We now introduce the \emph{Repeated Selection Model} (RSM), {\colorThree which aims to merge these two step into a more intuitive and realistic method.
    }
 This is a novel generative model for partial orders, which we regard as being of independent interest. 
It  includes earlier generative models of partial orders as special cases via a suitable choice of parameters.

Formally, a Repeated Selection Model over a set $A$ of $m$ items specifies a generator of a
random partial order on $A$ using three parameters:
\begin{itemize}
\item A \emph{reference ranking} $\sigma$, which is a total order on
  $A$.
\item A \emph{selection probability} $\Pi$ that defines, for all
  $i=1,\dots,m$ and $j=1,\dots,m-i+1$, a probability $\Pi(i,j)\in[0,1]$
  such that for all $i$, we have that $\sum_{j=1}^{m-i+1}\Pi(i,j)=1$.
\item A \emph{preference probability}
  $p:\{1,\dots,m\}\rightarrow[0,1]$.
\end{itemize}

Intuitively, RSM repeatedly selects a random item (according to the
probability defined by $\Pi$), and for each selected item, randomly
selects whether or not to include a preference over each of the items
that have not been selected so far (according to the probability
defined by $p$).  More formally, the random partial order $P$ is
generated as follows. Let $\tau$ be a listing of the items in the
order of $\sigma$. 
\begin{enumerate}
    \item Starting with an empty partial order $P$, repeat the following 
for $i=1,\dots,m$:

\begin{itemize}
\item Select a random number $j\in\{i,\dots,m-i+1\}$ with the
  probability $\Pi(i,j)$. 
\item Let $a$ be the item of $\tau$ at position $j$. 
%\item 
Remove $a$ from $\tau$. 
\item For every remaining item $a'$ in $\tau$, add to $P$ the
  preference $a\succ a'$ with the probability $p(i)$.
\end{itemize}
\item {\colorThree Take the transitive closure of $P$.} 
\end{enumerate}

\begin{figure}[t]
    \centering
    %\includegraphics[scale=0.475]{figures/ACM_TDS/RSM/RSM_HardnessTime_TDSphi.pdf}
    %\includegraphics[scale=0.475]{figures/ACM_TDS/RSM/RSM_HardnessTime_TDSdensity.pdf}
    \includegraphics[scale=0.475]{figures/RSM_fit/RSM_Gehrlein_TDS.pdf}
    %\includegraphics[scale=0.475]{figures/ACM_TDS/RSM/RSM_Hardness_TDS.pdf}
\vspace{-0.5cm}
  \caption{Density distribution of RSM, compared to two poset generation methods from Gehrlein~\cite{gehrlein1986methods}.}
 % \vspace{-0.3cm}
  \label{fig:RSM_eval_gehrlein}
\end{figure}

\theo{I'm not sure the below example is relevant, we can remove it or we can add a small figures which show the process in the example} \julia{Yes, definitely better to add a figure.  The example is too verbose.}
{
\colorThree
We illustrate RSM's methodology using an example having the following parameters: $m = 3$ candidates, $\sigma = (A,B,C)$, $p = (0.5,0.2,0)$ and $\phi = 0.2$ which gives us the following probability matrix (see Theorem~\ref{thm:RSM_Mallows}) : 
\[
\Pi = 
\begin{pmatrix}
0.81 & 0.16 & 0.03 \\
0.83 & 0.17 & 0 \\
1 & 0 & 0
\end{pmatrix}
\]
\begin{enumerate}
    \item We start with $P = \{\}$ and $\tau = \sigma =(A,B,C)$.  A candidate in $\tau$ is selected using the probability distribution $\Pi(1,*)$:
    \begin{itemize}
        \item Say, we select $B$ as our first candidate. 
        \item The candidates that remain in $\tau$ are $A$ and $C$. 
        \item As $p(1) = 0.5$, the pair $(B,A)$ is added to the ranking with a probability $0.5$, and so is the pair $(B,C)$. 
        \item Let's say both pairs are added to the ranking, we have $P = \{ (B,A),(B,C) \}$ and $\tau = (A,C)$.
    \end{itemize}
    \item We now select the second candidate. We repeat the above step using the probabilities from $\Pi(2,*)$:
    \begin{itemize}
        \item We select $A$ and add the pair $(A,C)$ to $P$ with probability $p(2) = 0.2$ and do not add it with probability $0.8$.
        \item We do not add it, so the profile remains $P = \{ (B,A),(B,C) \}$ and $tau = (C)$.
    \end{itemize}
     \item Finally, as there is only one remaining candidate in $\tau$, there is no need to add any more pairs to $P$ and we output $P = \{ (B,A),(B,C) \}$.
\end{enumerate}
}

As discussed earlier, we can replicate earlier generative models of partial orders as special cases via a suitable choice of parameters. For illustration, $p= (1,...,1,0,...,0)$ with $k$ ones  will generate a top-truncated partial order, 
%(with a total order on the top-$k$ items),
whereas $p=(0,...,0,1,...,1)$ with $k$ ones will generate a partial chain over a subset of $k$ items. Moreover, a uniform $p$ gives rise to the generative model referred to as \emph{Method 1} of Gehrlein~\cite{gehrlein1986methods}.  {\colorThree
Finally, %it is interesting to we note that
we can also simulate a Mallows model with RSM.
\begin{theorem} \label{thm:RSM_Mallows}
If
$\Pi_{i,j} = \frac{\phi^{j-1}}{\sum^{m-i+1}_{k=1}\phi^{k-1}}$ and
$\forall i, p(i)=1$, then RSM is the Mallows model of $\sigma$ and $\phi$ generated using the Kandall-Tau distance.
\end{theorem}

%\kunal{pi gives the distribution, p gives the full ranking.}

%\kunal{proof is in 2 parts: first line is to show that p gives the full ranking. The following part is to show that the distribution of ranking generated with RSM follows the distribution of ranking generated by Mallows with sigma and phi. equating the the probability of getting a particular ranking from rsm and from mallows. equal probability means that the distribution is the same. in turn, this means that rsm can replicate a mallows model.}


\begin{proof}
This is a two-part proof: (1) we show that the parameter $\forall i, p(i)=1$ returns a complete ranking. (2) Given that we get a complete ranking, we show that the  distribution of a voting profile generated using RSM is same as the  distribution of a voting profile generated using Mallows' model with $\sigma$ and $\phi$. More specifically, we equate the probability of getting a particular ranking from RSM and from mallows, and show that equal probability implies that the distribution is the same.

\paragraph{Part 1:} It is easily seen that we can obtain a complete ranking by using the condition $\forall i, p(i) = 1$ as every pair of candidate is added to the partial order.

\paragraph{Part 2:} Proof by induction showing that we can obtain a Mallows model using the RSM:
\begin{itemize}
    \item Base case: $m = 1$ candidate: this holds as there is only one ranking.
    \item Let's suppose that $m > 1$ and that the condition is true for $m-1$. Let $\sigma$ be the reference ranking, $\rho$ the ranking obtained with RSM, and $\rho_1$ the candidate selected in the first step of the algorithm. We denote$\sigma_{-\rho_1}$ the subranking of $\sigma$ with $c_1$ removed. By induction, the probability to obtain the permutation $\rho_{2..m}$ 
    %(\kunal{rho is the ranking we get using the rsm, rho' is ranking remaining after removal of c1.} \kunal{probability of getting a subranking using rsm = prob of getting subranking using mallows.}) 
     of $\sigma_{-\rho_1}$ is
    \[
    \mathbb{P}(\rho_{2..m}|\phi,\sigma_{-\rho_1}) = \frac{\phi^{d_{KT}(\rho_{2..m},\sigma_{-\rho_1})}}{Z(\phi,m-1)}
    \]
    with $Z(\phi,m-1)$ the normalization constant of Mallows with parameter $\phi$ and $m-1$ candidates. We easily see that 
    \[
    d_{KT}(\rho,\sigma) = d_{KT}(\rho_{2..m},\sigma_{-\rho_1}) + |\{~j~|~j >_{\sigma} c_1~\}| = d_{KT}(\rho_{2..m},\sigma_{-c_1}) + \sigma^{-1}(\rho_1) - 1
    \]
    However, the probability to select $\rho_1$ at the first step is given by 
    \[
    \Pi_{1,\sigma^{-1}(\rho_1)} = \frac{\phi^{\sigma^{-1}(\rho_1)-1}}{\sum^{m}_{k=1}\phi^{k-1}} = \frac{\phi^{\sigma^{-1}(\rho_1)-1}}{Z^*(\phi)}
    \]
    Finally, we find the probability of a Mallows:
    \begin{align*}
        \mathbb{P}(\rho|\sigma) &= \mathbb{P}(\rho_1 |\sigma)\times\mathbb{P}(\rho_{2..m} |\rho_1,\sigma) \\
        &= \frac{\phi^{\sigma^{-1}(\rho_1)-1}}{Z^*(\phi)}\times\frac{\phi^{d_{KT}(\rho_{2..m},\sigma_{-\rho_1})}}{Z(\phi,m-1)} 
        %&=\frac{\phi^{\sigma^{-1}(c_1)-1}\phi^{d_{KT}(\rho',\sigma_{-c_1})}}{Z_1\times Z'} \\
        =\frac{\phi^{d_{KT}(\rho_{2..m},\sigma_{-\rho_1})+\sigma^{-1}(\rho_1)-1}}{Z(\phi,m)}  
        =\frac{\phi^{d_{KT}(\rho,\sigma)}}{Z(\phi,m)}
    \end{align*}
    
\end{itemize}
    The proof by induction concludes and the theorem is proven.
\end{proof}
In our experiments, we use these values for $\Pi$ as it replicates Mallows model, which are known to be close to real world data \cite{marden,DBLP:conf/webdb/StoyanovichIP16}.
}

Figure~\ref{fig:RSM_eval_gehrlein} compares RSM with {\em Methods 1} and {\em 2} from Gehrlein~\cite{gehrlein1986methods}, by showing the empirical distribution of poset density, defined as $d = 2D / [m(m-1)]$, where $m$ is the number of items, and $D$ is the total number of preference pairs in $P$. {\colorThree We observe that the RSM generates partial orders over a wider range of densities as compared to other methods.}

\paragraph{Validation of RSM}  We conducted an experiment to verify that the Repeated Selection Model is sufficiently flexible to represent real partial voting profiles.  We extended the methods of Stoyanovich et al.~\cite{DBLP:conf/webdb/StoyanovichIP16} to fit a  RSM to the {\em dessert} dataset and to the {\em travel} dataset (both were described in Section~\ref{sec:poset:real}), observing the best fit with a RSM in both cases (Table~\ref{tab:nll}). 
\theo{Please note that we fit with one RSM, not a RSM Mix} 

{\colorThree 
More specifically, for each dataset, we compute the negative log-likelihood using the voters for whom we know both a full ranking $\rho$ and a partial ranking $T$:
\[
\mathcal{NLL} = -\frac{1}{n}\sum_{i}log(\mathbb{P}(T_i|\rho_i))
\]
Overall, RSM fits better to both the real world datasets when compared to the methods from Gehrlein's paper (lower negative log-likelihood values in Table~\ref{tab:nll} mean better fit \cite{DBLP:conf/webdb/StoyanovichIP16}).
% For the Dessert dataset, we isolate the voters for which we know both a full ranking $\rho$ and a partial ranking $T$ (around 110 voters) and we compute the negative log-likelihood:
% \[
% \mathcal{NLL} = -\frac{1}{n}\sum_{i}log(\mathbb{P}(T_i|\rho_i))
% \]
Synthetic methods fit the \emph{dessert} dataset better as compared to the \emph{travel} dataset because the latter contains partitioned preferences with missing candidates. The synthetic methods consider all the candidates appearing in its ranking for generating partial preferences making them a non-optimal fit to the \emph{travel} dataset. 
\begin{table}[]
    \centering
    \begin{tabular}{c|c|c|c}
    \toprule
        \multirow{2}{*}{\emph{Dataset}} & \multicolumn{3}{|c}{$\mathcal{NLL}$}  \\
        \cline{2-4}
         & \emph{Gehrlein 1} & \emph{Gehrlein 2} & \emph{RSM} \\
         \midrule\midrule
         \emph{Dessert (Sparse)} & $12.9$ & $14.7$ & $\mathbf{12.5}$\\ %\hline
         \midrule
         \emph{Dessert (Dense)} & $19.1$ & $19.8$& $\mathbf{18.7}$ \\ %\hline
         \midrule
         \emph{Travel} & $10.4$  &$10.4$ & $\mathbf{9.5}$\\ %\hline
    \bottomrule
    \end{tabular}
    \caption{Comparison of goodness-of-fit of synthetic data generation methods with real-world datasets. $\mathcal{NLL}$ stands for negative log-likelihood. Lower $\mathcal{NLL}$ value means better fit.}
    \label{tab:nll}
\end{table}
}


%We then quantified the correlations between the density distributions of the fitted models and those observed in the real datasets. We saw a very close fit, with Pearson's  $\rho = 0.89$ for the {\em travel} dataset, and $\rho = 0.96$ for {\em dessert}.

\paragraph{RSM Mix Datasets} 
Our third type of synthetic datasets,  \rsmm,
uses a mixture of three RSMs, each covering $\frac{1}{3}$ of the voters, with selection probability $\Pi_{i,j}$ corresponding to the Mallows model ($\phi=0.5$, randomly chosen $\sigma$ of size $m$). For each RSM, draw the preference probability $p(m)$ uniformly %at random 
from $[0,1]$ for each $m$.
%\end{itemize}

\eat{
\subsection{The Repeated Insertion Model and Mallows}
\par 
There exists several methods to generate full rankings. One of the most popular is the Mallows $\Phi$-model, with a reference ordering $\sigma$ and a parameter $\phi$~\cite{Mallows1957}. The probability to obtain a ranking $\phi$ is given by:
\begin{align}
    P(\rho_0|\sigma,\phi) = \frac{\phi^{d_{\textsc{kt}}(\sigma,\rho_0)}}{\sum_{\rho} \phi^{d_{\textsc{kt}}(\sigma,\rho)}}
\end{align}
where $d_{\textsc{kt}}$ is the \emph{Kendall-Tau distance} defined as the number of inversion between the two rankings :
\begin{align*}
    d_{\textsc{kt}}(\sigma,\rho) =
    |\{(i,j) | i < j ~\wedge ~& ((i >_{\sigma} j \wedge i <_{\rho} j) \\&\vee (i <_{\sigma} j \wedge i >_{\rho} j)) \}|
\end{align*}

When $\phi = 1$, we obtain a uniform distribution over the set of all possible rankings. When $\phi \rightarrow 0$ , the probability mass is concentrated around $\sigma$.
 
Almost 50 years later the \emph{Repeated Insertion Model (RIM)} was
introduced.  RIM generalizes Mallows and defines an efficient sampler
for complete rankings.  Our novel Repeated Selection Model (RSM)
generalized RIM to partially ordered sets, or posets.  In what
follows, we describe RSM, explain its relationship to the models
proposed by Gehrlein~\cite{gehrlein1986methods}, and show that it can
be fit to real datasets. 

\paragraph{The Repeated Selection Model (RSM)}  is a generative model. While in RIM we \emph{insert} every candidate one by one in the output ranking, in RSM we \emph{select} every candidate one by one to build our output ranking.  For instance, RSM  selects which candidate will be the first one in the output ranking. Then, the algorithm selects which candidate will be ranked in the second position. The process continues until every candidate have been selected. At the last step, the last remaining candidate takes the last position.

Formally, we have two inputs: a reference ranking $\sigma$ and a probability matrix $\Pi$. When we select the $i^th$ candidate at the \emph{step $i$}, we rank every remaining candidates in the order they are on $\sigma$ and we obtain a ranking $\sigma_i$ with $m-(i-1)$ candidates. Then, we select the $j^th$ candidate of $\sigma_i$ with probability $\Pi_{i,j}$.

With the above process, we obtain a full ranking. With $ \forall i, \forall j \le m - (i-1), \Pi_{i,j} = \frac{\phi^{j-1}}{\sum^{i}_{k=1}\phi^{k-1}}$, we obtain a Mallows model with parameters $(\sigma,\phi)$.

To enables to obtain partial orders, we add a third parameter: the \emph{probability vector} $p$. We initialize the partial order as an empty list of preference pairs $P$. At the \emph{step $i$}, when we select the $i^{th}$ candidate $c^i$, we know that every candidate which is not yet selected will be less well ranked than $c^i$. Consequently, for every remaining candidate $c'$, we independently add the preference pair $(c^i,c')$ to $P$ with a probability $p_i$.

With particular settings for $p$, we obtain known "partial order" models. For instance, with a uniform $p$, we simulate the random graph model, which is the Method 1 from Gehrlein \cite{}. With $p= (1,...,1,0,...,0)$, we will generate \emph{top-k} partial orders and with $p=(0,...,0,1,...,1)$ a \emph{partial chain} partial order.
 }
 
 
